Compete to Win: Enhancing Pseudo Labels for Barely-supervised Medical Image Segmentation

This study investigates barely-supervised medical image segmentation where only few labeled data, i.e., single-digit cases are available. We observe the key limitation of the existing state-of-the-art semi-supervised solution cross pseudo supervision is the unsatisfactory precision of foreground classes, leading to a degenerated result under barely-supervised learning. In this paper, we propose a novel Compete-to-Win method (ComWin) to enhance the pseudo label quality. In contrast to directly using one model's predictions as pseudo labels, our key idea is that high-quality pseudo labels should be generated by comparing multiple confidence maps produced by different networks to select the most confident one (a compete-to-win strategy). To further refine pseudo labels at near-boundary areas, an enhanced version of ComWin, namely, ComWin+, is proposed by integrating a boundary-aware enhancement module. Experiments show that our method can achieve the best performance on three public medical image datasets for cardiac structure segmentation, pancreas segmentation and colon tumor segmentation, respectively. The source code is now available at https://github.com/Huiimin5/comwin.

==> refs_old_short.tex <==

@book{ abelson-et-al:scheme,
  author = "Harold Abelson and Gerald~Jay Sussman and Julie Sussman",
  title = "Structure and Interpretation of Computer Programs",
  publisher = "MIT Press",
  address = "Cambridge, Massachusetts",
  year = "1985"
}

@inproceedings{ bgf:Lixto,
  author = "Robert Baumgartner and Georg Gottlob and Sergio Flesca",
  title = "Visual Information Extraction with {Lixto}",
  booktitle = "Proceedings of the 27th International Conference on Very Large Databases",
  pages = "119--128",
  publisher = "Morgan Kaufmann",
  address = "Rome, Italy",
  month = "September",
  year = "2001"
}

@article{ brachman-schmolze:kl-one,
  author = "Ronald~J. Brachman and James~G. Schmolze",
  title = "An overview of the {KL-ONE} knowledge representation system",
  journal = "Cognitive Science",
  volume = "9",
  number = "2",
  pages = "171--216",
  month = "April--June",
  year = "1985"
}

@article{ gottlob:nonmon,
  author = "Georg Gottlob",
  title = "Complexity results for nonmonotonic logics",
  journal = "Journal of Logic and Computation",
  volume = "2",
  number = "3",
  pages = "397--425",
  month = "June",
  year = "1992"
}

@article{ gls:hypertrees,
  author = "Georg Gottlob and Nicola Leone and Francesco Scarcello",
  title = "Hypertree Decompositions and Tractable Queries",
  journal = "Journal of Computer and System Sciences",
  volume = "64",
  number = "3",
  pages = "579--627",
  month = "May",
  year = "2002"
}

@article{ levesque:functional-foundations,
  author = "Hector~J. Levesque",
  title = "Foundations of a functional approach to knowledge representation",
  journal = "Artificial Intelligence",
  volume = "23",
  number = "2",
  pages = "155--212",
  month = "July",
  year = "1984"
}

@inproceedings{ levesque:belief,
  author = "Hector~J. Levesque",
  title = "A logic of implicit and explicit belief",
  booktitle = "Proceedings of the Fourth National Conference on Artificial Intelligence",
  publisher = "American Association for Artificial Intelligence",
  pages = "198--202",
  address = "Austin, Texas",
  month = "August",
  year = "1984"
}

@article{ nebel:jair-2000,
  author = "Bernhard Nebel",
  title = "On the compilability and expressive power of propositional planning formalisms",
  journal = "Journal of Artificial Intelligence Research",
  volume = "12",
  pages = "271--315",
  year = "2000"
}

 @misc{proceedings,
  author = {{IJCAI Proceedings}},
  title = {{IJCAI} Camera Ready Submission},
  howpublished = {\url{https://proceedings.ijcai.org/info}},
}


@inproceedings{yu2018recurrent,
  title={Recurrent saliency transformation network: Incorporating multi-stage visual cues for small organ segmentation},
  author={Yu, Qihang and Xie, Lingxi and Wang, Yan and Zhou, Yuyin and Fishman, Elliot K and Yuille, Alan L},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={8280--8289},
  year={2018}
}

@inproceedings{DBLP:conf/miccai/RothLFSLTS15,
  title={Deeporgan: Multi-level deep convolutional networks for automated pancreas segmentation},
  author={Roth, Holger R and Lu, Le and Farag, Amal and Shin, Hoo-Chang and Liu, Jiamin and Turkbey, Evrim B and Summers, Ronald M},
  booktitle={International conference on medical image computing and computer-assisted intervention},
  pages={556--564},
  year={2015},
  organization={Springer}
}
@article{simpson2019large,
  title={A large annotated medical image dataset for the development and evaluation of segmentation algorithms},
  author={Simpson, Amber L and Antonelli, Michela and Bakas, Spyridon and Bilello, Michel and Farahani, Keyvan and Van Ginneken, Bram and Kopp-Schneider, Annette and Landman, Bennett A and Litjens, Geert and Menze, Bjoern and others},
  journal={arXiv preprint arXiv:1902.09063},
  year={2019}
}
@inproceedings{DBLP:conf/3dim/MilletariNA16,
  title={V-net: Fully convolutional neural networks for volumetric medical image segmentation},
  author={Milletari, Fausto and Navab, Nassir and Ahmadi, Seyed-Ahmad},
  booktitle={2016 international conference on 3D vision (3DV)},
}
@inproceedings{DBLP:conf/miccai/YuWLFH19,
  title={Uncertainty-aware self-ensembling model for semi-supervised 3D left atrium segmentation},
  author={Yu, Lequan and Wang, Shujun and Li, Xiaomeng and Fu, Chi-Wing and Heng, Pheng-Ann},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={605--613},
  year={2019},
  organization={Springer}
}

 @inproceedings{luo2021urpc,
  title={Efficient semi-supervised gross target volume of nasopharyngeal carcinoma segmentation via uncertainty rectified pyramid consistency},
  author={Luo, Xiangde and Liao, Wenjun and Chen, Jieneng and Song, Tao and Chen, Yinan and Zhang, Shichuan and Chen, Nianyong and Wang, Guotai and Zhang, Shaoting},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={318--329},
  year={2021},
  organization={Springer}
}
@article{luo2021semi,
  title={Semi-Supervised Medical Image Segmentation through Dual-task Consistency},
  author={Luo, Xiangde and Chen, Jieneng and Song, Tao  and Wang, Guotai},
  journal={AAAI},
  year={2021}
}
@inproceedings{chen2021semi,
  title={Semi-supervised semantic segmentation with cross pseudo supervision},
  author={Chen, Xiaokang and Yuan, Yuhui and Zeng, Gang and Wang, Jingdong},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2613--2622},
  year={2021}
}
@article{tarvainen2017mean,
  title={Mean teachers are better role models: Weight-averaged consistency targets improve semi-supervised deep learning results},
  author={Tarvainen, Antti and Valpola, Harri},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}
@inproceedings{DBLP:conf/miccai/LiZH20,
  title={Shape-aware semi-supervised 3D semantic segmentation for medical images},
  author={Li, Shuailin and Zhang, Chuyu and He, Xuming},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={552--561},
  year={2020},
  organization={Springer}
}
@inproceedings{DBLP:conf/cvpr/VuJBCP19,
  title={Advent: Adversarial entropy minimization for domain adaptation in semantic segmentation},
  author={Vu, Tuan-Hung and Jain, Himalaya and Bucher, Maxime and Cord, Matthieu and P{\'e}rez, Patrick},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2517--2526},
  year={2019}
}
@inproceedings{DBLP:conf/miccai/ZhangYCFHC17,
  title={Deep adversarial networks for biomedical image segmentation utilizing unannotated images},
  author={Zhang, Yizhe and Yang, Lin and Chen, Jianxu and Fredericksen, Maridel and Hughes, David P and Chen, Danny Z},
  booktitle={International conference on medical image computing and computer-assisted intervention},
  pages={408--416},
  year={2017},
  organization={Springer}
}
@inproceedings{liu2021swin,
  title={Swin transformer: Hierarchical vision transformer using shifted windows},
  author={Liu, Ze and Lin, Yutong and Cao, Yue and Hu, Han and Wei, Yixuan and Zhang, Zheng and Lin, Stephen and Guo, Baining},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={10012--10022},
  year={2021}
}
@article{lucas2021barely,
  title={Barely-Supervised Learning: Semi-Supervised Learning with very few labeled images},
  author={Lucas, Thomas and Weinzaepfel, Philippe and Rogez, Gregory},
  journal={arXiv preprint arXiv:2112.12004},
  year={2021}
}
@inproceedings{bai2017semi,
  title={Semi-supervised learning for network-based cardiac MR image segmentation},
  author={Bai, Wenjia and Oktay, Ozan and Sinclair, Matthew and Suzuki, Hideaki and Rajchl, Martin and Tarroni, Giacomo and Glocker, Ben and King, Andrew and Matthews, Paul M and Rueckert, Daniel},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={253--260},
  year={2017},
  organization={Springer}
}
@inproceedings{ke2019dual,
  title={Dual student: Breaking the limits of the teacher in semi-supervised learning},
  author={Ke, Zhanghan and Wang, Daoye and Yan, Qiong and Ren, Jimmy and Lau, Rynson WH},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={6728--6736},
  year={2019}
}
@inproceedings{zhu2017deeply,
  title={Deeply-supervised CNN for prostate segmentation},
  author={Zhu, Qikui and Du, Bo and Turkbey, Baris and Choyke, Peter L and Yan, Pingkun},
  booktitle={2017 international joint conference on neural networks (IJCNN)},
  pages={178--184},
  year={2017},
  organization={IEEE}
}
@article{wang2019deeply,
  title={Deeply-supervised networks with threshold loss for cancer detection in automated breast ultrasound},
  author={Wang, Yi and Wang, Na and Xu, Min and Yu, Junxiong and Qin, Chenchen and Luo, Xiao and Yang, Xin and Wang, Tianfu and Li, Anhua and Ni, Dong},
  journal={IEEE transactions on medical imaging},
  volume={39},
  number={4},
  pages={866--876},
  year={2019},
  publisher={IEEE}
}
@inproceedings{lee2015deeply,
  title={Deeply-supervised nets},
  author={Lee, Chen-Yu and Xie, Saining and Gallagher, Patrick and Zhang, Zhengyou and Tu, Zhuowen},
  booktitle={Artificial intelligence and statistics},
  pages={562--570},
  year={2015},
  organization={PMLR}
}
@inproceedings{DBLP:conf/iclr/LaineA17,
  title={Temporal ensembling for semi-supervised learning},
  author={Samuli, Laine and Timo, Aila},
  booktitle={ICLR},
  volume={4},
  number={5},
  pages={6},
  year={2017}
}
@article{sajjadi2016regularization,
  title={Regularization with stochastic transformations and perturbations for deep semi-supervised learning},
  author={Sajjadi, Mehdi and Javanmardi, Mehran and Tasdizen, Tolga},
  journal={Advances in neural information processing systems},
  volume={29},
  pages={1163--1171},
  year={2016}
}
@inproceedings{DBLP:conf/miccai/HangFLYWCQ20,
  title={Local and global structure-aware entropy regularized mean teacher model for 3d left atrium segmentation},
  author={Hang, Wenlong and Feng, Wei and Liang, Shuang and Yu, Lequan and Wang, Qiong and Choi, Kup-Sze and Qin, Jing},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={562--571},
  year={2020},
  organization={Springer}
}
@inproceedings{DBLP:conf/miccai/FangL20,
  title={DMNet: difference minimization network for semi-supervised segmentation in medical images},
  author={Fang, Kang and Li, Wu-Jun},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={532--541},
  year={2020},
  organization={Springer}
}
@inproceedings{DBLP:conf/miccai/SedaiARJ0SWG19,
  title={Uncertainty guided semi-supervised segmentation of retinal layers in OCT images},
  author={Sedai, Suman and Antony, Bhavna and Rai, Ravneet and Jones, Katie and Ishikawa, Hiroshi and Schuman, Joel and Gadi, Wollstein and Garnavi, Rahil},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={282--290},
  year={2019},
  organization={Springer}
}
@inproceedings{DBLP:conf/iclr/ZouZZLBHP21,
  author    = {Yuliang Zou and
               Zizhao Zhang and
               Han Zhang and
               Chun{-}Liang Li and
               Xiao Bian and
               Jia{-}Bin Huang and
               Tomas Pfister},
  title     = {PseudoSeg: Designing Pseudo Labels for Semantic Segmentation},
  booktitle = {ICLR},
  year      = {2021},
  crossref  = {DBLP:conf/iclr/2021},
  url       = {https://openreview.net/forum?id=-TwO99rbVRu},
  timestamp = {Wed, 23 Jun 2021 17:36:39 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/ZouZZLBHP21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{zhou2019semi,
  title={Semi-supervised 3D abdominal multi-organ segmentation via deep multi-planar co-training},
  author={Zhou, Yuyin and Wang, Yan and Tang, Peng and Bai, Song and Shen, Wei and Fishman, Elliot and Yuille, Alan},
  booktitle={2019 IEEE Winter Conference on Applications of Computer Vision (WACV)},
}

@inproceedings{reiss2021every,
  title={Every annotation counts: Multi-label deep supervision for medical image segmentation},
  author={Rei{\ss}, Simon and Seibold, Constantin and Freytag, Alexander and Rodner, Erik and Stiefelhagen, Rainer},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  year={2021}
}



@inproceedings{DBLP:conf/colt/BlumM98,
  author    = {Avrim Blum and
               Tom M. Mitchell},
  editor    = {Peter L. Bartlett and
               Yishay Mansour},
  title     = {Combining Labeled and Unlabeled Data with Co-Training},
  booktitle = {Proceedings of the Eleventh Annual Conference on Computational Learning
               Theory, {COLT} 1998, Madison, Wisconsin, USA, July 24-26, 1998},
  pages     = {92--100},
  publisher = {{ACM}},
  year      = {1998},
  url       = {https://doi.org/10.1145/279943.279962},
  doi       = {10.1145/279943.279962},
  timestamp = {Fri, 25 Dec 2020 01:14:19 +0100},
  biburl    = {https://dblp.org/rec/conf/colt/BlumM98.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{oreiller2022head,
  title={Head and neck tumor segmentation in PET/CT: the HECKTOR challenge},
  author={Oreiller, Valentin and Andrearczyk, Vincent and Jreige, Mario and Boughdad, Sarah and Elhalawani, Hesham and Castelli, Joel and Valli{\`e}res, Martin and Zhu, Simeng and Xie, Juanying and Peng, Ying and others},
  journal={Medical image analysis},
  volume={77},
  pages={102336},
  year={2022},
  publisher={Elsevier}
}
@inproceedings{iantsen2020squeeze,
  title={Squeeze-and-excitation normalization for automated delineation of head and neck primary tumors in combined PET and CT images},
  author={Iantsen, Andrei and Visvikis, Dimitris and Hatt, Mathieu},
  booktitle={3D Head and Neck Tumor Segmentation in PET/CT Challenge},
  pages={37--43},
  year={2020},
  organization={Springer}
}
@inproceedings{DBLP:conf/colt/BlumM98,
  title={Combining labeled and unlabeled data with co-training},
  author={Blum, Avrim and Mitchell, Tom},
  booktitle={Proceedings of the eleventh annual conference on Computational learning theory},
  pages={92--100},
  year={1998}
}
@inproceedings{DBLP:conf/eccv/QiaoSZWY18,
  title={Deep co-training for semi-supervised image recognition},
  author={Qiao, Siyuan and Shen, Wei and Zhang, Zhishuai and Wang, Bo and Yuille, Alan},
  booktitle={Proceedings of the european conference on computer vision (eccv)},
  pages={135--152},
  year={2018}
}
@inproceedings{DBLP:conf/ijcai/ChenWGZ18,
  title={Tri-net for semi-supervised deep learning},
  author={Dong-DongChen, WeiWang and WeiGao, Zhi-HuaZhou},
  booktitle={Proceedings of twenty-seventh international joint conference on artificial intelligence},
  pages={2014--2020},
  year={2018}
}
@article{luo2021ctbct,
  title={Semi-Supervised Medical Image Segmentation via Cross Teaching between CNN and Transformer},
  author={Luo, Xiangde and Hu, Minhao and Song, Tao and Wang, Guotai and Zhang, Shaoting},
  booktitle={Medical Imaging with Deep Learning},
  year={2022}}
@article{bernard2018deep,
  title={Deep learning techniques for automatic MRI cardiac multi-structures segmentation and diagnosis: is the problem solved?},
  author={Bernard, Olivier and Lalande, Alain and Zotti, Clement and Cervenansky, Frederick and Yang, Xin and Heng, Pheng-Ann and Cetin, Irem and Lekadir, Karim and Camara, Oscar and Ballester, Miguel Angel Gonzalez and others},
  journal={IEEE transactions on medical imaging},
  volume={37},
  number={11},
  pages={2514--2525},
  year={2018},
  publisher={ieee}
}
@inproceedings{ronneberger2015u,
  title={U-net: Convolutional networks for biomedical image segmentation},
  author={Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas},
  booktitle={International Conference on Medical image computing and computer-assisted intervention},
  pages={234--241},
  year={2015},
  organization={Springer}
}

@article{cao2021swin,
  title={Swin-unet: Unet-like pure transformer for medical image segmentation},
  author={Cao, Hu and Wang, Yueyue and Chen, Joy and Jiang, Dongsheng and Zhang, Xiaopeng and Tian, Qi and Wang, Manning},
  journal={arXiv preprint arXiv:2105.05537},
  year={2021}
}
@inproceedings{yang2021st++,
  title={ST++: Make Self-training Work Better for Semi-supervised Semantic Segmentation},
  author={Yang, Lihe and Zhuo, Wei and Qi, Lei and Shi, Yinghuan and Gao, Yang},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  year={2022}
}
@inproceedings{shi2021semi,
  title={Semi-supervised Learning via Improved Teacher-Student Network for Robust 3D Reconstruction of Stereo Endoscopic Image},
  author={Shi, Hongkuan and Wang, Zhiwei and Lv, Jinxin and Wang, Yilang and Zhang, Peng and Zhu, Fei and Li, Qiang},
  booktitle={Proceedings of the 29th ACM International Conference on Multimedia},
  pages={4661--4669},
  year={2021}
}
@article{li2020transformation,
  title={Transformation-consistent self-ensembling model for semisupervised medical image segmentation},
  author={Li, Xiaomeng and Yu, Lequan and Chen, Hao and Fu, Chi-Wing and Xing, Lei and Heng, Pheng-Ann},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  volume={32},
  number={2},
  pages={523--534},
  year={2020},
  publisher={IEEE}
}
@inproceedings{li2018semi,
  title={Semi-supervised skin lesion segmentation via transformation consistent self-ensembling model},
  author={Li, Xiaomeng and Yu, Lequan and Chen, Hao and Fu, Chi-Wing and Heng, Pheng-Ann},
  booktitle=BMVC,
  year={2018}
}

@article{liu2022translation,
  title={Translation Consistent Semi-supervised Segmentation for 3D Medical Images},
  author={Liu, Yuyuan and Tian, Yu and Wang, Chong and Chen, Yuanhong and Liu, Fengbei and Belagiannis, Vasileios and Carneiro, Gustavo},
  journal={arXiv preprint arXiv:2203.14523},
  year={2022}
}

